Privacy Violations in Election Results

After an election, should election officials release a copy of each anonymous ballot? Some policymakers have championed public disclosure to counter distrust, but others worry that it might undermine ballot secrecy. We introduce the term vote revelation to refer to the linkage of a vote on an anonymous ballot to the voter's name in the public voter file, and detail how such revelation could theoretically occur. Using the 2020 election in Maricopa County, Arizona, as a case study, we show that the release of individual ballot records would lead to no revelation of any vote choice for 99.83% of voters as compared to 99.95% under Maricopa's current practice of reporting aggregate results by precinct and method of voting. Further, revelation is overwhelmingly concentrated among the few voters who cast provisional ballots or federal-only ballots. We discuss the potential benefits of transparency, compare remedies to reduce or eliminate privacy violations, and highlight the privacy-transparency tradeoff inherent in all election reporting.

==> tables/SI/tab-snyder_ecdf.tex <==
\begin{tabular}{rcccccc}
\toprule
 &  & \multicolumn{5}{c}{Voters per 100,000 in units of size:} \\ 
\cmidrule(lr){3-7}
Reporting Unit & Unique units & 1 & $\le 2$ & $\le 5$ & $\le 10$ & $\le 30$\\ 
\midrule\addlinespace[2.5pt]
Precinct & $8,001$ & $0$ & $1$ & $5$ & $12$ & $49$ \\ 
Ballot Style & $4,498$ & $1$ & $2$ & $6$ & $13$ & $46$ \\ 
Precinct $\times$ Ballot Style & $12,465$ & $3$ & $7$ & $16$ & $34$ & $117$ \\ 
Ballot Equivalent & $28,004$ & $10$ & $23$ & $67$ & $158$ & $559$ \\ 
\emph{... only mail method} & $10,173$ & $4$ & $8$ & $20$ & $43$ & $191$ \\ 
\emph{... only in-person method} & $14,787$ & $10$ & $24$ & $71$ & $174$ & $828$\\ 
\emph{... only provisional method} & $3,042$ & $422$ & $983$ & $3,022$ & $7,096$ & $15,991$\\ 
\bottomrule
\end{tabular}

==> tables/tb4_descrip/tab-ecdf_prec_stat.tex <==
743 & 0 & 0 & 0 & 1 & 3


==> tables/tb4_descrip/tab-ecdf_precstyl_stat.tex <==
1,741 & 1 & 4 & 34 & 124 & 358


==> tables/tb4_descrip/tab-ecdf_styl_stat.tex <==
381 & 0 & 0 & 2 & 5 & 13


==> tables/tb4_descrip/tab-ecdf_stylmethE_stat.tex <==
1,722 & 2 & 8 & 47 & 143 & 319


==> tables/tb4_descrip/tab-ecdf_stylmethI_stat.tex <==
1,369 & 126 & 256 & 469 & 657 & 1,530


==> tables/tb4_descrip/tab-ecdf_stylmethV_stat.tex <==
1,306 & 5,357 & 12,649 & 34,124 & 66,731 & 97,661


==> tables/tb4_descrip/tab-ecdf_stylmeth_stat.tex <==
4,397 & 28 & 65 & 182 & 381 & 705

